Insights from the Future for Continual Learning

Continual learning aims to learn tasks sequentially, with (often severe) constraints on the storage of old learning samples, without suffering from catastrophic forgetting. In this work, we propose prescient continual learning, a novel experimental setting, to incorporate existing information about the classes, prior to any training data. Usually, each task in a traditional continual learning setting evaluates the model on present and past classes, the latter with a limited number of training samples. Our setting adds future classes, with no training samples at all. We introduce Ghost Model, a representation-learning-based model for continual learning using ideas from zero-shot learning. A generative model of the representation space in concert with a careful adjustment of the losses allows us to exploit insights from future classes to constraint the spatial arrangement of the past and current classes. Quantitative results on the AwA2 and aP\&Y datasets and detailed visualizations showcase the interest of this new setting and the method we propose to address it.

==> reorganization.tex <==
=> Big picture
- Reunion Zero Shot + Incremental Learning
- On veut pas vendre du zeroshot learning. On l'utilise comme outil, mais c'est pas du tout le but de notre papier. On est avant tout en continual learning.

- Possible parce que on est dans un espace de representation / representation learning



- Travailler le modele en abstract (generateur, ghost features, etc) avant de preciser les intances concrete de la solution

- On veut pas non plus vendre en prio le fait qu'on "balance accuracy from past, current, and future classes". 'accuracy des futures est plutôt pas ouf. On veut faire le mieux possible sur l'ensemble, et surtout on veut que l'information des futures aide à ne pas abimer past & current. Genre dans mon toy model, on voit que les "insights" ont permis d'éviter un oubli des anciennes classes au profit des nouvelles.


=> Context Incremental
    - Zero Shot => Ghost
    - Contexte evolutive => Ghost arrive => Passe a pas ghost ensuite
    - Comment on contrains l'apprentissage avec le ghost
        Eq.4 => directement sur le classifier
        Lpod => loss distillation partie eviter cathastrophical learning
        Lreg => partie feature space / SVM Eq. 6 ou 7 ou 9 etc.

    - Loss de regularization en plus

    3.1. motivation
    3.2. basic model => archi complete?
    3.3. zero shot learning modelling
    3.4. Loss Eq.4 => Classification Loss with
    3.5. Regularization Loss for Learning => Partie

- Eq. 5 permettre de mettre a jour les centres/representants de classe
- le vues
- le passées
- les futurs (ghost)

- Eq. 1
- Quel est la procedure de mise-à-jour des thetas
- C'est different pour present / passé / futur (ghost)

- Peut-etre mettre le theta explicite en Eq. 5





==> tables/old_cheat.tex <==
\begin{table}
\caption{Comparison of \textit{generated} ghost features vs. \textit{actual} features extracted from future classes'\,samples with PODNet on AwA2 and aP\&Y.}
\label{tab:generated_vs_real}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
 \toprule
& \multicolumn{2}{c}{AwA2}            & \multicolumn{2}{c}{aP\&Y }        \\
 &  \multicolumn{2}{c}{25 classes + 5 $\times$ 5 classes} &  \multicolumn{2}{c}{16 classes + 8 $\times$ 2 classes} \\
Features & Continual & Final & Continual & Final\\
\midrule
\textit{None} & 62.92 \std 0.12 & 77.63 \std 0.06 & 58.64 \std 0.66 & 57.80 \std 0.97\\
Generated / Ghost  & \textbf{68.46 \std 0.47} & \textbf{79.08 \std 0.53} & \textbf{62.73 \std 0.60} & \textbf{63.30 \std 0.98}\\
Actual / From data & 67.65 \std 0.50 & 78.83 \std 0.31 & 61.88 \std 0.52 & 61.70 \std 0.26\\
\midrule
Actual / pixels level & 72.94 \std 0.25 & 84.60 \std 0.28 & 63.81 \std 0.29 & 68.03 \std 1.42\\
Oracle  & --- & 95.40 \std 0.02 & --- & 97.40 \std 0.30\\
\bottomrule
\end{tabular}
\end{table}

==> tables/qualitative_podflat.tex <==
\begin{table*}
\caption{Ghosts results on AwA2 and aP\&Y with \cite{hou2019ucir}'s Less-Forget distillation.}
\label{tab:awa2-apy-podflat}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
 \toprule
 & \multicolumn{2}{c}{AwA2, 25 classes + 5 classes $\times$ 5 classes} & \multicolumn{2}{c}{aP\&Y, 16 classes + 8 $\times$ 2 classes} \\
  & Avg & Acc & Avg & Acc\\
\midrule
UCIR \cite{hou2019ucir}                                                 & 54.80 \std 0.40 & 67.07 \std 0.81 & 43.42 \std 0.21 & 42.23 \std 1.34\\
%\,\,+ Zeroshot                                          & 56.96 \std 0.53 & 67.07 \std 0.81 & 45.72 \std 0.54 & 42.60 \std 0.85\\
\,\,+ $\mcL_\text{NCA-ghost}$                   & \textbf{57.88 \std 0.27} & \textbf{67.43 \std 0.08} & 50.23 \std 0.29 & 44.17 \std 1.48\\
\,\,+ $\mcL_\text{NCA-ghost}$ + $\mcL_\text{svm-reg}$ & 57.75 \std 0.42 & 66.50 \std 0.82 & \textbf{50.91 \std 0.56} & \textbf{45.97 \std 0.26} \\
\,\,+ $\mcL_\text{svm-reg}$                  & \tbd & \tbd & \tbd & \tbd\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/qualitative_small_first_step.tex <==
\begin{table}
\caption{Ghosts results on AwA2 with \cite{douillard2020podnet}'s POD distillation, with a smaller first step.}
\label{tab:awa2-apy-pod-512-smallfirststep}
\centering
\begin{tabular}{@{}l|cc@{}}
 \toprule
 & \multicolumn{2}{c}{AwA2, 10 classes + 4 $\times$ 10 classes}\\
 %\cmidrule(l{0pt}r{4pt}){2-4} \cmidrule(l{4pt}r{4pt}){5-7} \cmidrule(l{4pt}r{4pt}){8-9}
  & Continual Accuracy & Last Accuracy\\
\midrule
Base                                        & \tbd & \tbd\\
\,\,+ $\mcL_\text{NCA-ghost}$                     & \tbd & \tbd\\
\,\,+ $\mcL_\text{NCA-ghost}$ + $\mcL_\text{svm-reg}$   & \tbd & \tbd\\
%\,\,+ $\mcL_\text{svm-reg}$                        & \tbd & \tbd\\
\bottomrule
\end{tabular}
\end{table}

==> tables/quantitative_pod.tex <==
\begin{table*}[httb!]
\caption{Ghosts results on AwA2 with \cite{douillard2020podnet}'s POD distillation.}
\label{tab:awa2-512-zeroshot}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
 \toprule
 & \multicolumn{2}{c|}{40 classes + 5 $\times$ 2 classes} & \multicolumn{2}{c}{25 classes + 5 $\times$ 5 classes} \\
  & Avg & Acc & Avg & Acc\\
\midrule
PODNet \cite{douillard2020podnet}                                                    & 82.84 $\pm$ 0.10 & 84.70 $\pm$ 0.10 & 62.92 \std 0.12 & 77.63 \std 0.06\\
%\,\,+ Zeroshot                                             & 83.59 $\pm$ 0.45 & 84.70 $\pm$ 0.10 & 66.28 \std 0.71 & 77.63 \std 0.06\\
\,\,+ $\mcL_\text{NCA-ghost}$                     & \textbf{84.99 $\pm$ 0.17} & \textbf{86.57 $\pm$ 0.49} & 68.31 \std 0.36 & 78.70 \std 0.46\\
\,\,+ $\mcL_\text{NCA-ghost}$ + $\mcL_\text{svm-reg}$    & 84.47 \std 0.15 & 85.73 \std 0.40 & \textbf{68.32 \std 0.35} & \textbf{79.37 \std 0.64}\\
%+ Zeroshot + eq.\ref{eq:nca-ghost} + eq.\ref{eq:plc}    & 84.78  & 86.60 & 68.03 $\pm$ 0.13 & 79.16 $\pm$ 0.40\\
%+ Zeroshot + eq.\ref{eq:nca-ghost} + eq.\ref{eq:plc} + eq.\ref{eq:svm}    & \tbd & \tbd & \tbd & \tbd\\
\,\,+ $\mcL_\text{svm-reg}$                           & 83.62 \std 0.19 & 85.40 \std 0.61 & 66.94 \std 0.13 & 77.83 \std 0.91\\


%\midrule
%Oracle       & --- & 95.50 & --- & \tbd & --- & 87.20 & --- & \tbd\\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[httb!]
\caption{Ghosts results on aP\&Y with \cite{douillard2020podnet}'s POD distillation.}
\label{tab:apy-512-zeroshot}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
 \toprule
 & \multicolumn{2}{c|}{20 classes + 6 $\times$ 2 classes} & \multicolumn{2}{c}{16 classes + 8 $\times$ 2 classes} \\
  & Avg & Acc & Avg & Acc\\
\midrule
PODNet \cite{douillard2020podnet}                                                                    & 67.57 \std 0.41 & 65.23 \std 0.5 & 58.64 \std 0.66 & 57.80 \std 0.97\\
%\,\,+ Zeroshot                                                              & 66.95 \std 0.61 & 65.23 \std 0.5 & 60.20 \std 0.55 & 57.80 \std 0.97\\
\,\,+ $\mcL_\text{NCA-ghost}$                                      & 68.80 \std 0.98 & 67.93 \std 1.24 & 62.08 \std 0.25 & 62.47 \std 0.40\\
\,\,+ $\mcL_\text{NCA-ghost}$ + $\mcL_\text{svm-reg}$                    & \textbf{69.02 \std 0.46} & \textbf{67.97 \std 0.60} & \textbf{62.73 \std 0.60} & \textbf{63.30 \std 0.98}\\
\,\,+  $\mcL_\text{svm-reg}$                                            & \tbd & \tbd & 60.34 \std 0.36 & 57.83 \std 1.31\\
%\midrule
%Oracle       & --- & 95.50 & --- & \tbd & --- & 87.20 & --- & \tbd\\
\bottomrule
\end{tabular}
\end{table*}


==> tables/quantitative_pod_seen.tex <==
\begin{table}[tb]
\caption{Ghosts results on AwA2 and aP\&Y with \cite{douillard2020podnet}'s POD distillation, evaluated only on seen classes.}
\label{tab:awa2-apy-pod-512-nozeroshot}
\centering
\begin{tabular}{@{}l|cc|cc@{}}
 \toprule
 & \multicolumn{2}{c}{AwA2, 25 classes + 5 $\times$ 5 classes} & \multicolumn{2}{c}{aP\&Y, 16 classes + 8 $\times$ 2 classes} \\
 %\cmidrule(l{0pt}r{4pt}){2-4} \cmidrule(l{4pt}r{4pt}){5-7} \cmidrule(l{4pt}r{4pt}){8-9}
  & Avg & Acc & Avg & Acc\\
\midrule
Base                                        & 85.49 \std 0.23 & 78.67 \std 0.49 & \tbd & \tbd\\
\,\,+ $\mcL_\text{NCA-ghost}$                     & \tbd & \tbd & \tbd & \tbd\\
\,\,+ $\mcL_\text{NCA-ghost}$ + $\mcL_\text{svm-reg}$   & \tbd & \tbd & \tbd & \tbd\\
\,\,+ $\mcL_\text{svm-reg}$                           & \tbd & \tbd & \tbd & \tbd\\
\bottomrule
\end{tabular}
\end{table}
